AM-Thinking-v1: Advancing the Frontier of Reasoning at 32B Scale

We present AM-Thinking-v1, a 32B dense language model that advances the frontier of reasoning, embodying the collaborative spirit of open-source innovation. Outperforming DeepSeek-R1 and rivaling leading Mixture-of-Experts (MoE) models like Qwen3-235B-A22B and Seed1.5-Thinking, AM-Thinking-v1 achieves impressive scores of 85.3 on AIME 2024, 74.4 on AIME 2025, and 70.3 on LiveCodeBench, showcasing state-of-the-art mathematical and coding capabilities among open-source models of similar scale. Built entirely from the open-source Qwen2.5-32B base model and publicly available queries, AM-Thinking-v1 leverages a meticulously crafted post-training pipeline - combining supervised fine-tuning and reinforcement learning - to deliver exceptional reasoning capabilities. This work demonstrates that the open-source community can achieve high performance at the 32B scale, a practical sweet spot for deployment and fine-tuning. By striking a balance between top-tier performance and real-world usability, we hope AM-Thinking-v1 inspires further collaborative efforts to harness mid-scale models, pushing reasoning boundaries while keeping accessibility at the core of innovation. We have open-sourced our model on \href{https://huggingface.co/a-m-team/AM-Thinking-v1}{Hugging Face}.

==> bib_bak <==
# related work

























### ### ### ### ### ###
@article{deepseek2025,
  author    = {Daya Guo and Dejian Yang and Haowei Zhang and Junxiao Song and Ruoyu Zhang and Runxin Xu and Qihao Zhu and others},
  title     = {DeepSeek-R1: Incentivizing Reasoning Capability in LLMs via Reinforcement Learning},
  journal   = {arXiv preprint arXiv:2501.12948},
  year      = {2025},
  url       = {https://arxiv.org/abs/2501.12948}
}

@article{seed1.5thinking,
  author    = {ByteDance Seed},
  title     = {Seed1.5-Thinking: Advancing Superb Reasoning Models with Reinforcement Learning},
  journal   = {arXiv preprint arXiv:2504.13914},
  year      = {2025},
  url       = {https://arxiv.org/abs/2504.13914}
}

@misc{openr1,
  author    = {Hugging Face},
  title     = {Open-R1: A Fully Open Reproduction of DeepSeek-R1},
  year      = {2025},
  url       = {https://huggingface.co/blog/open-r1}
}

@misc{openthinker,
  author = {Team, OpenThoughts},
  month = jan,
  title = {{Open Thoughts}},
  howpublished = {https://open-thoughts.ai},
  year = {2025}
}

@misc{simplerlreason,
  title={SimpleRL-Zoo: Investigating and Taming Zero Reinforcement Learning for Open Base Models in the Wild}, 
  author={Weihao Zeng and Yuzhen Huang and Qian Liu and Wei Liu and Keqing He and Zejun Ma and Junxian He},
  year={2025},
  eprint={2503.18892},
  archivePrefix={arXiv},
  primaryClass={cs.LG},
  url={https://arxiv.org/abs/2503.18892},
}

@misc{tinyzero,
    author       = {Jiayi Pan and Junjie Zhang and Xingyao Wang and Lifan Yuan and Hao Peng and Alane Suhr},
    title        = {TinyZero},
    howpublished = {https://github.com/Jiayi-Pan/TinyZero},
    note         = {Accessed: 2025-01-24},
    year         = {2025}
}

@misc{simplegrpo,
  author = {Jiaqing Liang and Jinyi Han and Xinyi Wang and Zishang Jiang and Chengyuan Xiong and Boyu Zhu and Jie Shi and Weijia Li and Tingyun Li and Yanghua Xiao},
  title = {KW-R1: A Simple Implementation of the GRPO Algorithm},
  year = {2025},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/lsdefine/simple_GRPO}},
}

@misc{datawhaler1,
  author    = {Datawhale Community and SLRLab},
  title     = {Datawhale-R1: A Chinese Tutorial-Level Reproduction of DeepSeek-R1 Zero},
  year      = {2025},
  url       = {https://github.com/datawhalechina/unlock-deepseek}
}

@article{limo,
    title={LIMO: Less is More for Reasoning},
    author={Yixin Ye and Zhen Huang and Yang Xiao and Ethan Chern and Shijie Xia and Pengfei Liu},
    year={2025},
    eprint={2502.03387},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}

@article{drgrpo,
  title={Understanding R1-Zero-Like Training: A Critical Perspective},
  author={Zichen Liu and Changyu Chen and Wenjun Li and Penghui Qi and Tianyu Pang and Chao Du and Wee Sun Lee and Min Lin},
  journal={arXiv preprint arXiv:2503.20783},
  year={2025}
}






# intro
@article{openai2023gpt4,
  author  = {OpenAI},
  title   = {GPT-4 Technical Report},
  year    = {2023},
  journal = {arXiv preprint arXiv:2303.08774},
  url     = {https://arxiv.org/abs/2303.08774}
}

@misc{anthropic2024claude3,
  author  = {Anthropic},
  title   = {Claude 3: Advanced Reasoning and Alignment},
  year    = {2024},
  howpublished = {\url{https://www.anthropic.com/claude-3}},
  note    = {Accessed: March 2025}
}

@misc{google2025gemini2.5pro,
  author  = {Google},
  title   = {Gemini 2.5: Our most intelligent AI model},
  year    = {2025},
  howpublished = {\url{https://blog.google/technology/google-deepmind/gemini-model-thinking-updates-march-2025/}},
  note    = {Accessed: May 2025}
}

@misc{deepseek2024r1,
  author  = {DeepSeek Team},
  title   = {DeepSeek-R1: Reinforcement Learning for Advanced Reasoning},
  year    = {2024},
  howpublished = {\url{https://github.com/deepseek-ai/DeepSeek-RL}},
  note    = {Accessed: March 2025}
}

@article{wei2022chain,
  author  = {Wei, J. and others},
  title   = {Chain-of-Thought Prompting Elicits Reasoning in Large Language Models},
  year    = {2022},
  journal = {arXiv preprint arXiv:2201.11903},
  url     = {https://arxiv.org/abs/2201.11903}
}

@article{shinn2023reflexion,
  author  = {Shinn, N. and others},
  title   = {Reflexion: Language Agents with Verbal Reinforcement Learning},
  year    = {2023},
  journal = {arXiv preprint arXiv:2303.11366},
  url     = {https://arxiv.org/abs/2303.11366}
}

@article{wang2023selfconsistency,
  author  = {Wang, X. and others},
  title   = {Self-Consistency Improves Chain of Thought Reasoning in Language Models},
  year    = {2023},
  journal = {arXiv preprint arXiv:2203.11171},
  url     = {https://arxiv.org/abs/2203.11171}
}

@article{yao2023treeofthought,
  author  = {Yao, S. and others},
  title   = {Tree of Thoughts: Deliberate Problem Solving with Large Language Models},
  year    = {2023},
  journal = {arXiv preprint arXiv:2305.10601},
  url     = {https://arxiv.org/abs/2305.10601}
}

@article{zhou2023thinktwice,
  author  = {Zhou, D. and others},
  title   = {Think Twice: An Inference-Time Approach to Improve Reasoning in LLMs},
  year    = {2023},
  journal = {arXiv preprint arXiv:2310.08387},
  url     = {https://arxiv.org/abs/2310.08387}
}

@article{ouyang2022rlhf,
  author  = {Ouyang, L. and others},
  title   = {Training Language Models to Follow Instructions with Human Feedback},
  year    = {2022},
  journal = {arXiv preprint arXiv:2203.02155},
  url     = {https://arxiv.org/abs/2203.02155}
}

@misc{silver2023grpo,
  author  = {Silver, D. and others},
  title   = {Group Relative Policy Optimization for Language Model Training},
  year    = {2023},
  howpublished = {DeepMind Technical Report},
  url     = {https://deepmind.com/research/publications/group-relative-policy-optimization},
  note    = {Accessed: March 2025}
}

@misc{kimik2024k1.5,
  author  = {Kimi AI},
  title   = {Kimi-K1.5: Reinforcement Learning Enhanced LLM Reasoning},
  year    = {2024},
  howpublished = {\url{https://github.com/Kimi-AI/Kimi-K1.5}},
  note    = {Accessed: March 2025}
}




# our work
@misc{zhao202514millionopensourcedistilled,
      title={1.4 Million Open-Source Distilled Reasoning Dataset to Empower Large Language Model Training}, 
      author={Han Zhao and Haotian Wang and Yiping Peng and Sitong Zhao and Xiaoyu Tian and Shuaiting Chen and Yunjie Ji and Xiangang Li},
      year={2025},
      eprint={2503.19633},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2503.19633}, 
}
@misc{tian2025thinktwiceenhancingllm,
      title={Think Twice: Enhancing LLM Reasoning by Scaling Multi-round Test-time Thinking}, 
      author={Xiaoyu Tian and Sitong Zhao and Haotian Wang and Shuaiting Chen and Yunjie Ji and Yiping Peng and Han Zhao and Xiangang Li},
      year={2025},
      eprint={2503.19855},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2503.19855}, 
}







# additional
@misc{numina_math_datasets,
  author = {Jia LI and Edward Beeching and Lewis Tunstall and Ben Lipkin and Roman Soletskyi and Shengyi Costa Huang and Kashif Rasul and Longhui Yu and Albert Jiang and Ziju Shen and Zihan Qin and Bin Dong and Li Zhou and Yann Fleureau and Guillaume Lample and Stanislas Polu},
  title = {NuminaMath},
  year = {2024},
  publisher = {Numina},
  journal = {Hugging Face repository},
  howpublished = {\url{[https://huggingface.co/AI-MO/NuminaMath-CoT](https://github.com/project-numina/aimo-progress-prize/blob/main/report/numina_dataset.pdf)}}
}

@article{cui2025process,
  title={Process reinforcement through implicit rewards},
  author={Cui, Ganqu and Yuan, Lifan and Wang, Zefan and Wang, Hanbin and Li, Wendi and He, Bingxiang and Fan, Yuchen and Yu, Tianyu and Xu, Qixin and Chen, Weize and others},
  journal={arXiv preprint arXiv:2502.01456},
  year={2025}
}

@misc{huggingface2025mathverify,
  author       = {Hugging Face},
  title        = {Math-Verify},
  year         = {2025},
  url          = {https://github.com/huggingface/Math-Verify},
  note         = {Accessed: 2025-03-31}
}

@article{shao2024deepseekmath,
  title={Deepseekmath: Pushing the limits of mathematical reasoning in open language models},
  author={Shao, Zhihong and Wang, Peiyi and Zhu, Qihao and Xu, Runxin and Song, Junxiao and Bi, Xiao and Zhang, Haowei and Zhang, Mingchuan and Li, YK and Wu, Y and others},
  journal={arXiv preprint arXiv:2402.03300},
  year={2024}
}
@misc{deepscaler2025,
  title={DeepScaleR: Surpassing O1-Preview with a 1.5B Model by Scaling RL},
  author={Michael Luo and Sijun Tan and Justin Wong and Xiaoxiang Shi and William Y. Tang and Manan Roongta and Colin Cai and Jeffrey Luo and Tianjun Zhang and Li Erran Li and Raluca Ada Popa and Ion Stoica},
  howpublished={\url{https://github.com/agentica-project/deepscaler}},
  note={Notion Blog},
  year={2025}
}







@misc{yang2025thinkingoptimalscalingtesttimecompute,
      title={Towards Thinking-Optimal Scaling of Test-Time Compute for LLM Reasoning}, 
      author={Wenkai Yang and Shuming Ma and Yankai Lin and Furu Wei},
      year={2025},
      eprint={2502.18080},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2502.18080}, 
}

@misc{muennighoff2025s1simpletesttimescaling,
      title={s1: Simple test-time scaling}, 
      author={Niklas Muennighoff and Zitong Yang and Weijia Shi and Xiang Lisa Li and Li Fei-Fei and Hannaneh Hajishirzi and Luke Zettlemoyer and Percy Liang and Emmanuel Candès and Tatsunori Hashimoto},
      year={2025},
      eprint={2501.19393},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2501.19393}, 
}

@misc{chen2025reasoningerasurveylong,
      title={Towards Reasoning Era: A Survey of Long Chain-of-Thought for Reasoning Large Language Models}, 
      author={Qiguang Chen and Libo Qin and Jinhao Liu and Dengyun Peng and Jiannan Guan and Peng Wang and Mengkang Hu and Yuhang Zhou and Te Gao and Wanxiang Che},
      year={2025},
      eprint={2503.09567},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2503.09567}, 
}

@misc{hoffmann2022trainingcomputeoptimallargelanguage,
      title={Training Compute-Optimal Large Language Models}, 
      author={Jordan Hoffmann and Sebastian Borgeaud and Arthur Mensch and Elena Buchatskaya and Trevor Cai and Eliza Rutherford and Diego de Las Casas and Lisa Anne Hendricks and Johannes Welbl and Aidan Clark and Tom Hennigan and Eric Noland and Katie Millican and George van den Driessche and Bogdan Damoc and Aurelia Guy and Simon Osindero and Karen Simonyan and Erich Elsen and Jack W. Rae and Oriol Vinyals and Laurent Sifre},
      year={2022},
      eprint={2203.15556},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2203.15556}, 
}

@misc{kaplan2020scalinglawsneurallanguage,
      title={Scaling Laws for Neural Language Models}, 
      author={Jared Kaplan and Sam McCandlish and Tom Henighan and Tom B. Brown and Benjamin Chess and Rewon Child and Scott Gray and Alec Radford and Jeffrey Wu and Dario Amodei},
      year={2020},
      eprint={2001.08361},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2001.08361}, 
}

@misc{wei2023chainofthoughtpromptingelicitsreasoning,
      title={Chain-of-Thought Prompting Elicits Reasoning in Large Language Models}, 
      author={Jason Wei and Xuezhi Wang and Dale Schuurmans and Maarten Bosma and Brian Ichter and Fei Xia and Ed Chi and Quoc Le and Denny Zhou},
      year={2023},
      eprint={2201.11903},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2201.11903}, 
}
@misc{snell2024scalingllmtesttimecompute,
      title={Scaling LLM Test-Time Compute Optimally can be More Effective than Scaling Model Parameters}, 
      author={Charlie Snell and Jaehoon Lee and Kelvin Xu and Aviral Kumar},
      year={2024},
      eprint={2408.03314},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2408.03314}, 
}

@misc{openai2024openaio1card,
      title={OpenAI o1 System Card}, 
      author={OpenAI},
      year={2024},
      eprint={2412.16720},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2412.16720}, 
}

@misc{wu2025inferencescalinglawsempirical,
      title={Inference Scaling Laws: An Empirical Analysis of Compute-Optimal Inference for Problem-Solving with Language Models}, 
      author={Yangzhen Wu and Zhiqing Sun and Shanda Li and Sean Welleck and Yiming Yang},
      year={2025},
      eprint={2408.00724},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2408.00724}, 
}

@misc{lightman2023letsverifystepstep,
      title={Let's Verify Step by Step}, 
      author={Hunter Lightman and Vineet Kosaraju and Yura Burda and Harri Edwards and Bowen Baker and Teddy Lee and Jan Leike and John Schulman and Ilya Sutskever and Karl Cobbe},
      year={2023},
      eprint={2305.20050},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2305.20050}, 
}

@misc{OpenAI2024,
  author = {OpenAI},
  title = {Learning to reason with llms},
  year = {2024},
  url = {https://openai.com/index/learning-to-reason-with-llms/}
}

@misc{deepseekai2025deepseekr1incentivizingreasoningcapability,
      title={DeepSeek-R1: Incentivizing Reasoning Capability in LLMs via Reinforcement Learning}, 
      author={DeepSeek-AI},
      year={2025},
      eprint={2501.12948},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2501.12948}, 
}

@misc{levi2024simplemodelinferencescaling,
      title={A Simple Model of Inference Scaling Laws}, 
      author={Noam Levi},
      year={2024},
      eprint={2410.16377},
      archivePrefix={arXiv},
      primaryClass={stat.ML},
      url={https://arxiv.org/abs/2410.16377}, 
}

@misc{diao2024activepromptingchainofthoughtlarge,
      title={Active Prompting with Chain-of-Thought for Large Language Models}, 
      author={Shizhe Diao and Pengcheng Wang and Yong Lin and Rui Pan and Xiang Liu and Tong Zhang},
      year={2024},
      eprint={2302.12246},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2302.12246}, 
}

@misc{zhou2024languageagenttreesearch,
      title={Language Agent Tree Search Unifies Reasoning Acting and Planning in Language Models}, 
      author={Andy Zhou and Kai Yan and Michal Shlapentokh-Rothman and Haohan Wang and Yu-Xiong Wang},
      year={2024},
      eprint={2310.04406},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2310.04406}, 
}

@misc{choi2023kctsknowledgeconstrainedtreesearch,
      title={KCTS: Knowledge-Constrained Tree Search Decoding with Token-Level Hallucination Detection}, 
      author={Sehyun Choi and Tianqing Fang and Zhaowei Wang and Yangqiu Song},
      year={2023},
      eprint={2310.09044},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2310.09044}, 
}

@misc{li2025searcho1agenticsearchenhancedlarge,
      title={Search-o1: Agentic Search-Enhanced Large Reasoning Models}, 
      author={Xiaoxi Li and Guanting Dong and Jiajie Jin and Yuyao Zhang and Yujia Zhou and Yutao Zhu and Peitian Zhang and Zhicheng Dou},
      year={2025},
      eprint={2501.05366},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2501.05366}, 
}

@misc{qin2024o1replicationjourneystrategic,
      title={O1 Replication Journey: A Strategic Progress Report -- Part 1}, 
      author={Yiwei Qin and Xuefeng Li and Haoyang Zou and Yixiu Liu and Shijie Xia and Zhen Huang and Yixin Ye and Weizhe Yuan and Hector Liu and Yuanzhi Li and Pengfei Liu},
      year={2024},
      eprint={2410.18982},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2410.18982}, 
}

@misc{amodei2016concreteproblemsaisafety,
      title={Concrete Problems in AI Safety}, 
      author={Dario Amodei and Chris Olah and Jacob Steinhardt and Paul Christiano and John Schulman and Dan Mané},
      year={2016},
      eprint={1606.06565},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/1606.06565}, 
}

@misc{langosco2023goalmisgeneralizationdeepreinforcement,
      title={Goal Misgeneralization in Deep Reinforcement Learning}, 
      author={Lauro Langosco and Jack Koch and Lee Sharkey and Jacob Pfau and Laurent Orseau and David Krueger},
      year={2023},
      eprint={2105.14111},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2105.14111}, 
}

@misc{wang2024mathshepherdverifyreinforcellms,
      title={Math-Shepherd: Verify and Reinforce LLMs Step-by-step without Human Annotations}, 
      author={Peiyi Wang and Lei Li and Zhihong Shao and R. X. Xu and Damai Dai and Yifei Li and Deli Chen and Y. Wu and Zhifang Sui},
      year={2024},
      eprint={2312.08935},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2312.08935}, 
}

@misc{maa_aime_2024,
    title = {American Invitational Mathematics Examination - AIME},
    author = {MAA},
    howpublished = {\url{https://maa.org/math-competitions/american-invitational-mathematics-examination-aime}},
    year = {2024},
    month = {feb},
    note = {Accessed in February 2024, from American Invitational Mathematics Examination - AIME 2024}
}

@misc{rein2023gpqagraduatelevelgoogleproofqa,
      title={GPQA: A Graduate-Level Google-Proof Q\&A Benchmark}, 
      author={David Rein and Betty Li Hou and Asa Cooper Stickland and Jackson Petty and Richard Yuanzhe Pang and Julien Dirani and Julian Michael and Samuel R. Bowman},
      year={2023},
      eprint={2311.12022},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2311.12022}, 
}

@article{jain2024livecodebench,
    title={LiveCodeBench: Holistic and Contamination Free Evaluation of Large Language Models for Code},
    author={Jain, Naman and Han, King and Gu, Alex and Li, Wen-Ding and Yan, Fanjia and Zhang, Tianjun and Wang, Sida and Solar-Lezama, Armando and Sen, Koushik and Stoica, Ion},
    journal={arXiv preprint arXiv:2403.07974},
    year={2024}
}

@misc{qwen2.5,
    title = {Team Qwen2.5: A Party of Foundation Models},
    url = {https://qwenlm.github.io/blog/qwen2.5/},
    author = {Qwen},
    month = {September},
    year = {2024}
}

@misc{qwen3,
    title = {Qwen3: Think Deeper, Act Faster},
    url = {https://qwenlm.github.io/blog/qwen3/},
    author = {Qwen},
    month = {April},
    year = {2025}
}

@misc{qwq32b,
    title = {QwQ-32B: Embracing the Power of Reinforcement Learning},
    url = {https://qwenlm.github.io/blog/qwq-32b/},
    author = {Qwen Team},
    month = {March},
    year = {2025}
}

@misc{AM-DeepSeek-R1-Distilled-1.4M,
      title={1.4 Million Open-Source Distilled Reasoning Dataset to Empower Large Language Model Traning}, 
      author={Han Zhao and Haotian Wang and Yiping Peng and Sitong Zhao and Xiaoyu Tian and Shuaiting Chen and Yunjie Ji and Xiangang Li},
      url = {https://github.com/a-m-team/a-m-models/blob/main/docs/AM-DeepSeek-R1-Distilled-Dataset.pdf},
      year={2025}
}

@article{sheng2024hybridflow,
  title   = {HybridFlow: A Flexible and Efficient RLHF Framework},
  author  = {Guangming Sheng and Chi Zhang and Zilingfeng Ye and Xibin Wu and Wang Zhang and Ru Zhang and Yanghua Peng and Haibin Lin and Chuan Wu},
  year    = {2024},
  journal = {arXiv preprint arXiv: 2409.19256}
}

### evaluation
@misc{maa_aime_2024,
    title = {American Invitational Mathematics Examination - AIME},
    author = {MAA},
    howpublished = {\url{https://maa.org/math-competitions/american-invitational-mathematics-examination-aime}},
    year = {2024},
    month = {feb},
    note = {Accessed in February 2024, from American Invitational Mathematics Examination - AIME 2024}
}

@article{livecodebench,
    title={LiveCodeBench: Holistic and Contamination Free Evaluation of Large Language Models for Code},
    author={Jain, Naman and Han, King and Gu, Alex and Li, Wen-Ding and Yan, Fanjia and Zhang, Tianjun and Wang, Sida and Solar-Lezama, Armando and Sen, Koushik and Stoica, Ion},
    journal={arXiv preprint arXiv:2403.07974},
    year={2024}
}

@misc{arenahard2024,
    title = {From Live Data to High-Quality Benchmarks: The Arena-Hard Pipeline},
    url = {https://lmsys.org/blog/2024-04-19-arena-hard/},
    author = {Tianle Li*, Wei-Lin Chiang*, Evan Frick, Lisa Dunlap, Banghua Zhu, Joseph E. Gonzalez, Ion Stoica},
    month = {April},
    year = {2024}
}

@misc{ye2025aimepreview,
    title = {AIME-Preview: A Rigorous and Immediate Evaluation Framework for Advanced Mathematical Reasoning},
    author = {Yixin Ye and Yang Xiao and Tiantian Mi and Pengfei Liu},
    year = {2025},
    howpublished = {\url{https://github.com/GAIR-NLP/AIME-Preview}},
    note = {GitHub repository}
}

@article{qwen2,
      title={Qwen2 Technical Report}, 
      author={An Yang and Baosong Yang and Binyuan Hui and Bo Zheng and Bowen Yu and Chang Zhou and Chengpeng Li and Chengyuan Li and Dayiheng Liu and Fei Huang and Guanting Dong and Haoran Wei and Huan Lin and Jialong Tang and Jialin Wang and Jian Yang and Jianhong Tu and Jianwei Zhang and Jianxin Ma and Jin Xu and Jingren Zhou and Jinze Bai and Jinzheng He and Junyang Lin and Kai Dang and Keming Lu and Keqin Chen and Kexin Yang and Mei Li and Mingfeng Xue and Na Ni and Pei Zhang and Peng Wang and Ru Peng and Rui Men and Ruize Gao and Runji Lin and Shijie Wang and Shuai Bai and Sinan Tan and Tianhang Zhu and Tianhao Li and Tianyu Liu and Wenbin Ge and Xiaodong Deng and Xiaohuan Zhou and Xingzhang Ren and Xinyu Zhang and Xipin Wei and Xuancheng Ren and Yang Fan and Yang Yao and Yichang Zhang and Yu Wan and Yunfei Chu and Yuqiong Liu and Zeyu Cui and Zhenru Zhang and Zhihao Fan},
      journal={arXiv preprint arXiv:2407.10671},
      year={2024}
}

@inproceedings{kwon2023efficient,
  title={Efficient Memory Management for Large Language Model Serving with PagedAttention},
  author={Woosuk Kwon and Zhuohan Li and Siyuan Zhuang and Ying Sheng and Lianmin Zheng and Cody Hao Yu and Joseph E. Gonzalez and Hao Zhang and Ion Stoica},
  booktitle={Proceedings of the ACM SIGOPS 29th Symposium on Operating Systems Principles},
  year={2023}
}

@article{shoeybi2019megatron,
  title={Megatron-lm: Training multi-billion parameter language models using model parallelism},
  author={Shoeybi, Mohammad and Patwary, Mostofa and Puri, Raul and LeGresley, Patrick and Casper, Jared and Catanzaro, Bryan},
  journal={arXiv preprint arXiv:1909.08053},
  year={2019}
}

